Prediction-Based Task Assignment in Spatial Crowdsourcing (Technical Report)

Spatial crowdsourcing refers to a system that periodically assigns a number of location-based workers with spatial tasks nearby (e.g., taking photos or videos at some spatial locations). Previous works on the spatial crowdsourcing usually designed task assignment strategies that maximize some assignment scores, which are however only based on available workers/tasks in the system at the time point of assigning workers/tasks. These strategies may achieve local optimality, due to the neglect of future workers/tasks that may join the system. In contrast, in this paper, we aim to achieve "globally" optimal task assignments, by considering not only those present, but also future (via predictions), workers/tasks. Specifically, we formalize an important problem, namely prediction-based spatial crowdsourcing (PB-SC), which expects to obtain a "globally" optimal strategy for worker-and-task assignments, over both present and predicted task/worker locations, such that the total assignment quality score is maximized under the constraint of the traveling budget. In this paper, we design an effective grid-based prediction method to estimate spatial distributions of workers/tasks in the future, and then utilize the predicted ones in our procedure of task assignments. We prove that the PB-SC problem is NP-hard, and thus intractable. Therefore, we propose efficient approximate algorithms to tackle the PB-SC problem, including greedy and divide-and-conquer (D&C) approaches, which can efficiently assign workers to spatial tasks with high quality scores and low budget consumptions, by considering both current and future task/worker distributions. Through extensive experiments, we demonstrate the efficiency and effectiveness of our PB-SC processing approaches on real/synthetic data.

==> adaptive.tex <==
\section{The Adaptive Timing Determination Approach}
\label{sec:adaptive}

Up to now, we always assume that our PA-SC algorithms are conducted
for every round, for example, at timestamps $(p-1)$, $p$, $(p+1)$,
and so on, where one timestamp is a time unit (such as 1 second, or
1 minute). Note that, due to the time-varying workload of the
spatial crowdsourcing system (e.g., different numbers of
workers/tasks that may newly join the system), it is not
time-efficient to find assignment strategies for each timestamp.
Inspired by this, in this section, we will discuss how to adaptively
determine the best time to apply our PA-SC algorithm, and then start
a new round.

Specifically, at the current round at timestamp $p$, our goal is to
determine whether the current timestamp $p$ is the best time that we
apply the PA-SC algorithm, or we should wait for the next round at
timestamp $(p+1)$ to obtain good assignments.

In order to decide the best timing, we will take into account two
timing conditions related two factors/measures, respectively, that
is, the quality score of assignments and the efficiency of the PA-SC
algorithm. We would perform the PA-SC algorithm, as long as one of
the two conditions is satisfied (whichever is earlier).



\subsection{The Timing Condition of the Quality Score}

%\noindent \textbf{Adaptive Condition of Quality Score.}

The first timing condition is related to the quality score. Assume
that, at the current timestamp $p$, the system has $m_p$ available
spatial tasks in set $W_p$, and $n_p$ available workers in set
$T_p$. Without loss of generality, we denote $opt\_I_p$ as an
optimal worker-and-task assignment set, by using an optimal PA-SC
algorithm over sets $W_p$ and $T_p$ at timestamp $p$.




Similarly, at timestamp $(p+1)$ (in the next round), there are
$m_{p+1}$ predicted tasks in set $W_{p+1}$ and $n_{p+1}$ predicted
workers in set $T_{p+1}$ that may newly join the system (after
timestamp $p$). If we have already applied the PA-SC algorithm at
timestamp $p$, then at timestamp $(p+1)$, we have the available
worker set, $W'_{p+1} (= W_p \cup W_{p+1} - W(opt\_I_p))$, and
available task set, $T'_{p+1} (= T_p \cup T_{p+1} -T(opt\_I_p))$,
where $W(opt\_I_p)$ and $T(opt\_I_p)$ are worker and task sets in
optimal assignment set $opt\_I_p$, respectively.







Moreover, denote $W$ and $T$ as worker and task sets, respectively,
that are available at both timestamps $p$ and $(p+1)$. That is, we
have $W=W_p \cup W_{p+1}$ and $T=T_p \cup T_{p+1}$.



Next, assume that function $\mathbb{Q}_p(W_p,T_p)$ returns the total
quality score of optimal assignments in $opt\_I_p$ at timestamp $p$;
function $\mathbb{Q}_{p+1}(W'_{p+1},$ $T'_{p+1})$ outputs the total
quality score of optimal assignments over the remaining workers in
set $W'_{p+1}$ and tasks in set $T'_{p+1}$ (after performing the
assignment at timestamp $p$); and function $\mathbb{Q}_{p, (p+1)}(W,
T)$ obtains the total quality score of optimal assignments over
current/predicted workers and tasks at both timestamps $p$ and
$(p+1)$.



\noindent {\bf The Quality Score Condition.} Our timing condition
w.r.t. the total quality score is as follows. We will start to
perform the PA-SC algorithm at timestamp $p$, if it holds
that:\vspace{-2ex}

{\scriptsize
    \begin{eqnarray}
\mathbb{Q}_p(W_p,T_p) + \mathbb{Q}_{p+1}(W'_{p+1}, T'_{p+1}) >
\mathbb{Q}_{p, (p+1)}(W, T). \label{eq:quality_adaptive_condition}
    \end{eqnarray}\vspace{-3ex}
}

Intuitively, Eq.~(\ref{eq:quality_adaptive_condition}) compares the
total quality score by performing the PA-SC algorithm at timestamps
$p$ and $(p+1)$ separately with that executing the PA-SC algorithm
over both current and predicted workers/tasks. If the former quality
score is higher than the latter one, then it implies that the
current timestamp $p$ is the best time to conduct the PA-SC
assignment algorithm.









\noindent {\bf The Estimation of Function $\mathbb{Q}_{p, (p+1)}(W,
T)$.} Next, we discuss how to estimate the value of $\mathbb{Q}_{p,
(p+1)}(W,$ $T)$, which is the (maximum possible) total quality score
of optimal assignment pairs $\langle \tilde{w_i},$
$\tilde{t_j}\rangle$, over both current and future workers/tasks
(i.e., $W$ and $T$).

Denote $P(\tilde{w_i})$ and $P(\tilde{t_j})$ as the probability that
a worker $\tilde{w_i}$ is assigned with some task at timestamp $p$,
and the probability that a task $t_j$ is assigned to some worker at
timestamp $p$, respectively. Note that, in a special case, if
$\tilde{w_i}$ and $\tilde{t_j}$ are current worker or task at
timestamp $p$, then it holds that $P(\tilde{w_i}) = P(\tilde{t_j})
=1$.


Let $\tilde{t_x}$ and $\tilde{w_x}$ be the task and worker that have
the highest quality scores for worker $\tilde{w_i}$ and task
$\tilde{t_j}$, respectively.

Then, we can estimate $\mathbb{Q}_{p, (p+1)}(W,$ $T)$ as
follows:\vspace{-2ex}

{\scriptsize
\begin{equation}
\mathbb{Q}_{p, (p+1)}(W,T)=\left\{
\begin{array}{ll}
\sum_{\tilde{w_i}\in W} P(\tilde{w_i}) \cdot \hat{p_{ix}} \cdot \hat{q_{ix}}, & |W| \leq |T| \\
\sum_{\tilde{t_j}\in T} P(\tilde{t_j}) \cdot \hat{p_{xj}} \cdot
\hat{q_{xj}}, & |W| > |T|
\end{array}
\right. \label{eq:Q_p_p+1}
\end{equation}
}

\noindent where $\hat{p_{ix}}$ (and $\hat{p_{xj}}$) is the existence
probability of the pair $\langle \tilde{w_i}, \tilde{t_x}\rangle$
(or $\langle \tilde{w_x}, \tilde{t_j}\rangle$), $\hat{q_{ix}}$ (and
$\hat{q_{xj}}$) is the total quality score of the pair (as defined
in Section \ref{subsec:statistics}), $P(\tilde{w_i}) =
\frac{|opt\_I_p|}{|W_p|}$, and $P(\tilde{t_j}) =
\frac{|opt\_I_p|}{|T_p|}$.

\noindent {\bf The Estimation of Function
$\mathbb{Q}_{p+1}(W'_{p+1}, T'_{p+1})$.} Similarly, we can obtain
the value of $\mathbb{Q}_{p+1}(W'_{p+1}, T'_{p+1})$
below:\vspace{-2ex}

{\scriptsize
\begin{eqnarray}
&&\mathbb{Q}_{p+1}(W'_{p+1}, T'_{p+1})\label{eq:Q_p+1}\\
&=&\left\{
\begin{array}{ll}
\sum_{\tilde{w_i}\in W'_{p+1}} P(\tilde{w_i}) \cdot \hat{p_{ix}} \cdot \hat{q_{ix}}, & |W'_{p+1}| \leq |T'_{p+1}| \\
\sum_{\tilde{t_j}\in T'_{p+1}} P(\tilde{t_j}) \cdot \hat{p_{xj}}
\cdot \hat{q_{xj}}, & |W'_{p+1}| > |T'_{p+1}|
\end{array}
\right.\notag
\end{eqnarray}\vspace{-3ex}
}

\noindent where $|W'_{p+1}| =  (1-P(\tilde{w_i})) \cdot |W_p| +
|W_{p+1}|$ and $|T'_{p+1}| =  (1-P(\tilde{t_j})) \cdot |T_p| +
|T_{p+1}|$.

%{\bf (Peng, please double check the correctness of formula above.)}

%{\bf
%For a worker $w_i$ at timestamp $p$, the probability that he/she is
%assigned to some task is given by:
%\begin{equation}
%f(w_i)=\left\{
%\begin{array}{ll}
%\frac{|I_{k}|}{|W_{k}|}, & \text{$w_i$ comes in $p$} \\
%\frac{|I_{k}|}{|W_{k}|}(1-\frac{|I_{k}|}{|W_{k}|}), & \text{$w_i$ comes in $p-1$}
%\end{array}
%\right.
%\label{eq:select_worker_probability}
%\end{equation}
%
%
%\noindent where $I_{k}$ is the assignment instance set in last round and $W_k$ is the total number of workers in last round.
%
%For a task $t_j$ at timestamp $p$, the probability that it is assigned with some worker is given by:
%\begin{equation}
%g(t_j)=\left\{
%\begin{array}{ll}
%\frac{|I_k|}{T_k}, & \text{$t_i$ comes in $p$} \\
%\frac{|I_{k}|}{|T_{k}|}(1-\frac{|I_{k}|}{|T_{k}|}), & \text{$t_i$ comes in $p-1$}
%\end{array}
%\right.
%\label{eq:select_task_probability}
%\end{equation}
%
%\noindent where $I_k$ is the assignment instance set in last round and $T_k$ is the total number of tasks in last round.
%
%Then, for timestamp $p$, the upper bound of the total quality score for given a set of workers $W$ and a set of $T$ is estimated as:
%
%\begin{equation}
%\mathbb{Q}_{p}(W,T)=\left\{
%\begin{array}{ll}
%\sum_{w_i\in W}f(w_i)g(t_x)\widehat{p_{ix}}q_{ix}, & |W| \leq |T| \\
%\sum_{t_j\in W}f(w_x)g(t_j)\widehat{p_{xj}}q_{xj}, & |W| > |T|
%\end{array}
%\right.
%\label{eq:quality_upper}
%\end{equation}
%
%\noindent where $t_x$ and $w_x$ is the task and worker that has the
%highest quality score for worker $w_i$ and task $t_j$ respectively;
%$\widehat{p_{ix}}$ is the probability that the pair between worker
%$w_i$ and task $t_x$ is valid (defined in subsection
%\ref{subsec:statistics}).
%
%
%We consider two successive timestamp $p$ and $p+1$. When we consider
%whether to start a next round to assign workers to tasks at
%timestamp $p$, we can check the condition:
%
%\begin{eqnarray}
%&&\mathbb{Q}_p(W_p,T_p) + \mathbb{Q}_{p+1}(W_{p} \cup W_{p+1},T_p \cup T_{p+1}) \notag\\
%&>& \mathbb{Q}_{p}(W_{p} \cup W_{p+1},T_p \cup T_{p+1})
%\label{eq:quality_adaptive_condition}
%\end{eqnarray}
%
%\noindent where, $W_p$ and $T_p$ are the total workers and tasks in timestamp $p$; $W_{p+1}$ and $T_{p+1}$ are the predicted workers and tasks comes in timestamp $p+1$.
%
%If the condition \ref{eq:quality_adaptive_condition} holds, which
%means start a round at current timestamp can have a upper bound
%higher than start a round at the next timestamp, we can start a
%round of assignment in current timestamp $p$.
%
%}


\subsection{The Timing Condition of the Efficiency}

%\noindent \textbf{Adaptive Condition of the Efficiency.}


The second timing condition is related to the efficiency. That is,
we need to decide whether it is more efficient to conduct the PA-SC
algorithm (e.g., greedy or D\&C) at timestamps $p$ and $(p+1)$
separately (twice), or perform the PA-SC algorithm once over
current/predicted workers/tasks at both timestamps $p$ and $(p+1)$.

\noindent {\bf The Efficiency Condition.} Similar to the quality
score condition, assume that we have three functions,
$\mathbb{E}_p(W_p,T_p)$, $\mathbb{E}_{p+1}(W'_{p+1},$ $T'_{p+1})$,
and $\mathbb{E}_{p, (p+1)}(W, T)$, where $\mathbb{E}_p(W_p,T_p)$ is
the time cost of assignments over $W_p$ and $T_p$ at the current
timestamp $p$, $\mathbb{E}_{p+1}(W'_{p+1},$ $T'_{p+1})$ is the one
of assignments over sets $W'_{p+1}$ and $T'_{p+1}$, and
$\mathbb{E}_{p, (p+1)}(W, T)$ is the one of assignments over $W$ and
$T$ at both timestamps $p$ and $(p+1)$.



%{\bf (Peng, please discuss the three functions above.)}

Then, if we should perform the PA-SC algorithm at the current
timestamp $p$, if the efficiency condition holds that:\vspace{-2ex}

{\scriptsize
\begin{eqnarray}
\mathbb{E}_p(W_p,T_p) + \mathbb{E}_{p+1}(W'_{p+1}, T'_{p+1}) <
\mathbb{E}_{p, (p+1)}(W, T).
\label{eq:efficiency_condition}\vspace{-3ex}
\end{eqnarray}
}

\noindent {\bf The Function Estimations for the Greedy Algorithm.}
If we apply the greedy algorithm (in Section \ref{sec:greedy})
during the PA-SC processing, then we have the cost of the greedy
algorithm given as follows.

Assume that we consider the greedy algorithm over $n$ workers in
$W_p$ and $m$ tasks in $T_p$.\vspace{-2ex}

{\scriptsize
\begin{equation}
cost_{greedy}(W_p, T_p) = m\cdot n + h\big(3(m\cdot n)^2 + m +n\big)
+ h,
\end{equation}\vspace{-3ex}
}

\noindent where $m=|T_p|$, $n=|W_p|$, and $h$ = $\min\{|W_p|,
|T_p|\}$.

As a result, we have:

$\mathbb{E}_p(W_p,T_p) = cost_{greedy}(W_p, T_p)$,

$\mathbb{E}_{p+1}(W'_{p+1}, T'_{p+1}) = cost_{greedy}(W'_{p+1},
T'_{p+1})$, and

$\mathbb{E}_{p, (p+1)}(W, T) = cost_{greedy}(W, T)$.


\noindent {\bf The Function Estimations for the D\&C Algorithm.}
Similarly, the time cost, $cost_{D\&C} (W_p, T_p)$, of the D\&C
Algorithm can be given by Eq.~(\ref{eq:D&C_cost}). Thus, we have
functions in Eq.~(\ref{eq:quality_adaptive_condition}) below:


$\mathbb{E}_p(W_p,T_p) = cost_{D\&C}(W_p, T_p)$,

$\mathbb{E}_{p+1}(W'_{p+1}, T'_{p+1}) = cost_{D\&C}(W'_{p+1},
T'_{p+1})$, and

$\mathbb{E}_{p, (p+1)}(W, T) = cost_{D\&C}(W, T)$.


Therefore, as shown in line 2 of the framework (Figure
\ref{alg:framework}), we can check the timing conditions given by
Eqs.~(\ref{eq:quality_adaptive_condition}) and
(\ref{eq:efficiency_condition}), respectively, with respect to the
quality score and efficiency. If both conditions are not satisfied,
then we can skip the current round.



%
%
%{\bf (Peng, could you add the conditions and discussions to the two
%items above please?)\\
%
%
%We want to choose a good timestamp to start next round of assignment
%to minimize the computational cost of our proposed approaches,
%\textit{greedy} and \textit{divide-and-conquer}.
%
%For the computational cost of \textit{divide-and-conquer}, we can estimate it through Eq. \ref{eq:D&C_cost}, which needs three parameters: the number, $m$, of tasks, the number, $g$, of groups and the average number, $deg_t$, of valid workers for each task.  We can check this condition:
%
%\begin{eqnarray}
%&& cost_{D\&C}^{(p)}(m_p,g^{(p)}, deg_t^{(p)}) \notag\\
%&+& cost_{D\&C}^{(p+1)}(m'_p + m_{p+1},g^{(p+1)'}, deg_t^{(p+1)'}) \notag\\
%&>& cost_{D\&C}^{(p)}(m_p + m_{p+1},g^{(p+1)}, deg_t^{(p+1)})
%\label{eq:dc_adaptive_condition}
%\end{eqnarray}
%
%\noindent where $m_p$ is the number of tasks in timestamp $p$,$ g^{(p)}$ is the best estimated group number for timestamp $p$, and $deg_t^{(p)}$ is the average number of valid workers for each task in timestamp $p$. At the same time, $m'_p=(1-\frac{|I_{k}|}{|T_{k}|})m_p$, where $I_k$ is the assignment instance set in last round and $T_k$ is the total number of tasks in last round. $m_{p+1}$ is the number of tasks come in timestamp $p+1$. $deg_t^{(p+1)}$ can be calculated from the  current and predicted  workers and tasks, and $deg_t^{(p+1)'} = deg_t^{(p+1)} - \frac{|I_{k}|}{|W_{k}|}deg_t^{(p)}$. $g^{(p+1)}$ and $g^{(p)}$ can be estimated. If condition \ref{eq:dc_adaptive_condition} holds, we can start a round of assignment using the divide-and-conquer algorithm in the current timestamp $p$.
%
%Similarly, we can estimate the running cost of \textit{greedy} approach. For the greedy algorithm in Figure \ref{alg:greedy}, line 1 needs $O(mn)$ cost to find all the valid pairs. There are min\{$|W|, |T|$\}  iterations at most. For each iteration, lines 5-9 cost at most $2(mn)^2$. As the size of $S_p$ is at most $mn$, line 10 costs at most $(mn)^2$. To remove the related pairs of the selected pair $\langle \tilde{w_i}, \tilde{t_j}\rangle$, we at most remove $m+n$ pairs, then line 12 costs $m+n$. As the selected pairs are at most min\{$|W|, |T|$\}  pairs, line 13 needs at most min\{$|W|, |T|$\}. Thus, the cost of greedy is given by:
%
%\begin{equation}
%cost_{greedy} = mn + R\big(3(mn)^2 + m +n\big) + R
%\end{equation}
%
%\noindent where $R$ = min\{$|W|, |T|$\} . Similarly, we can have a checking condition for the greedy approach.
%
%\begin{eqnarray}
%&& cost_{greedy}^{(p)}(m_p,n_p) \notag\\
%&+& cost_{greedy}^{(p+1)}(m'_p + n'_p) \notag\\
%&>& cost_{greedy}^{(p)}(m_p + m_{p+1},n_p + n_{(p+1)})
%\label{eq:greedy_adaptive_condition}
%\end{eqnarray}
%
%\noindent where $m_p$ and $n_p$ are the numbers of tasks and workers in timestamp $p$ respectively.
%$m'_p=(1-\frac{|I_{k}|}{|T_{k}|})m_p$ and $n'_p=(1-\frac{|I_{k}|}{|W_{k}|})n_p$, where $I_k$ is the assignment instance set in last round and $T_k$ and $W_k$ are the total numbers of tasks and workers in last round respectively. $m_{p+1}$ and $n_{p+1}$ are the numbers of tasks and workers come in timestamp $p+1$ respectively. If condition \ref{eq:greedy_adaptive_condition} holds, we can start a round of assignment using the greedy algorithm in the current timestamp $p$.
%
%}


==> branchbound.tex <==

\newpage
\section*{Appendix}

\section{The Branch-and-Bound Approach}
\label{sec:branchbound}

In this section, we present the best-optimal-first branch-and-bound
approach ($BB$) for achieving the optimal assignment strategy. $BB$
maintains a current best assignment, which has the highest total
quality score among all the exploited nodes. When processing each
node, we first estimate the upper bound of the total quality score
with respect to the determined worker-and-task pairs and remaining
budget. If the upper bound is lower than the known highest total
quality score, we can safely prune the node. For a task of $k$ valid
workers, who can arrive at the task before its arrival deadline, it
can be assigned to any valid worker or postponed to the next round,
which is $(k+1)$ possible choices. With $m$ tasks and $n$ workers,
the search tree will have $m$ active levels and the search space
could be $(n+1)^m$ huge. Thus, an efficient method to calculate a
tight upper bound for each node of the searching space is
essentially important.

Figure \ref{fig:bb_example} shows the procedure of our $BB$ approach on an
example of 3 workers, $w_1 \sim w_3$, and 3 tasks, $t_1 \sim t_3$. The
corresponding quality scores and travel costs of valid worker-and-task
pairs are presented in Tables \ref{tab:travel_costs} and \ref{tab:travel_costs} respectively.
For example, the quality score of worker-and-task pair $\langle w_1, t_2\rangle$ is 1.
The circles with numbers indicates the expanding orders of the nodes. Here, each
node represents a valid situation of assignment under the constraints of budget and time.
The red star marker on the right top corner of a node indicates that a
best known total quality score was found. Meanwhile, the red cross marker on
the right top corner of a node indicates that the node is pruned.





\subsection{The Branching Procedure}
In this subsection, we introduce the procedure to expand a node in the search tree.
In the search tree, each node indicates a
situation of a possible assignment strategy. For a node $c$, it contains
its current quality score $c.score$,  current assigned worker-and-task pairs $c.I$,
remaining budget $c.budget$, upper bound of the total quality score $c.upperBound$ and maximum exploited task index number $c.taskIndex$.

Figure \ref{alg:bb_expand} shows the pseudo code of our TBC-SC branching
algorithm, namely TBC-SC\_Expand, which returns a set $O$ of the child nodes
of a given node $o$. We first initialize $O$ as an empty set (line 1). As our
branch-and-bound approach incrementally exploit $m$ tasks, to expand
the node $o$, we first obtain the next task $t_j$ to exploit for the next level (line 2).
Moreover, for this task $t_j$, we retrieve its valid workers $W$ from $S$, which does
not contain the workers have been assigned in previous levels (line 3).
Then, for each worker $w_i$ in the set $W$, we create a new node $o'$
indicating selecting worker $w_i$ to conduct task $t_j$ (line 5). Moreover,
we set the properties of node $o'$ based on the selected worker $w_i$ (lines 6-10).
Specifically, we use the procedure TBC-SC\_ComputeBound to estimate the
upper bound of the total quality score for node $o'$ (line 10). All the newly created nodes are added to the set $O$ (line 11). In addition, for the
situation where no worker is assigned to task $t_j$, we simply update the maximum
exploited task index value of node $o$ to $j$ and add $o$ to the set $O$ too (lines 12-13).
Finally, we return the child nodes set $O$ (line 14).


\begin{figure}[t]\centering
    \scalebox{0.48}[0.48]{\includegraphics{../figures/bb_example.eps}}\vspace{-1ex}
    \caption{\small An Example of Branch-And-Bound Approach.}\vspace{-1ex}
    \label{fig:bb_example}
\end{figure}


\begin{table}\vspace{-1ex}
    \parbox[b]{.4\linewidth}{
        \caption{\small Quality Scores}\label{tab:quality_scores}
        {\small\scriptsize\centering
            \begin{tabular}{l|lll}
                {\bf Workers}&\multicolumn{3}{c}{\textbf{Tasks}}\\
                \hline
                & {\bf   $t_1$} & {\bf   $t_2$}& {\bf   $t_3$}\\
                $w_1$& 3& 1& / \\
                $w_2$& 2& 4& 4\\
                $w_3$& / & /& 2\\
                \hline
            \end{tabular}
        }
        \vspace{-1ex}
    }
    \hfill\hspace{5ex}
    \parbox[b]{.4\linewidth}{
        \caption{\small Travel Costs}\label{tab:travel_costs}
            {\small\scriptsize\centering
                \begin{tabular}{l|lll}
                    {\bf Workers}&\multicolumn{3}{c}{\textbf{Tasks}}\\
                    \hline
                     & {\bf   $t_1$} & {\bf   $t_2$}& {\bf   $t_3$}\\

                    $w_1$& 1& 3& / \\
                    $w_2$& 3& 1& 5\\
                    $w_3$& / & /& 4\\
                    \hline
                \end{tabular}
            }
        \vspace{-1ex}
    }
    \vspace{-2ex}
\end{table}



\begin{figure}[ht]
    \begin{center}
        \begin{tabular}{l}
            \parbox{3.1in}{
                \begin{scriptsize} \vspace{-4ex}
                    \begin{tabbing}
                        12\=12\=12\=12\=12\=12\=12\=12\=12\=12\=12\=\kill
                        {\bf Procedure {\sf TBC-SC\_Expand}} \{ \\
                        \> {\bf Input:} a set of valid worker-and-task pairs $S$, and a node $c$\\
                        \> {\bf Output:} a set $O$ of child nodes of $o$\\
                        \> (1) \> \> $O = \emptyset$\\
                        \> (2) \> \> obtain the next unexploited task $t_j$ //the task with the biggest index number\\
                        \> (3) \> \> obtain a set $W$ of valid workers of $t_j$ //exclude workers have been assigned\\
                        \> (4) \> \> \textbf{foreach} worker $w_i$ in $W$\\
                        \> (5) \> \> \> create a new child node $o'$\\
                        \> (6) \> \> \> $o'.score$ = $o.score$ + $q_{ij}$\\
                        \> (7) \> \> \> $o'.budget$ = $o.budget$ - $c_{ij}$\\
                        \> (8) \> \> \> $o'.taskIndex$ = $j$\\
                        \> (9) \> \> \> $o'.I$ = $o.I + \langle w_i, t_j\rangle$\\
                        \> (10) \> \> \> $o'.upperBound$ = TBC-SC\_ComputeBound($o'$, $S$)\\
                        \> (11) \> \> \> $O$.add($o'$)\\
                        \> (12) \> \> $o.taskIndex=j$\\
                        \> (13) \> \> $O$.add($o$) //no worker is assigned to task $t_j$\\
                        \> (14) \> \>  \textbf{return} $O$\\
                        \}
                    \end{tabbing}
                \end{scriptsize}
            }
        \end{tabular}
    \end{center}\vspace{-8ex}
    \caption{\small The Expanding Algorithm.}
    \vspace{-3ex}
    \label{alg:bb_expand}
\end{figure}

\subsection{The Bounding Procedure}
In this subsection, we present a method to estimate the upper bound of the
quality score of a node in the search tree of our branch-and-bound approach.

For a worker-and-task pair $\langle w_i, t_j \rangle$, we define its quality
rate $qr_{ij}$ as follows:
\begin{equation}
qr_{ij}=\left\{
\begin{array}{ll}
q_{ij}/c_{ij}, & c_{ij} \neq 0\\
1, & c_{ij} = 0
\end{array}
\right.
\label{eq:quality_rate}
\end{equation}

Intuitively, selecting worker-and-task pairs with highest quality rates of
workers will lead to a highest total quality score. However, this process may be
unreachable as some tasks may be assigned with more than one worker. Here,
to estimate the upper bound of total quality score, we relax this constraint and
allow a task to be assigned with more than one worker. A worker is also allowed to assigned with more than one task.

\begin{figure}[ht]
    \begin{center}
        \begin{tabular}{l}
            \parbox{3.1in}{
                \begin{scriptsize} \vspace{-4ex}
                    \begin{tabbing}
                        12\=12\=12\=12\=12\=12\=12\=12\=12\=12\=12\=\kill
                        {\bf Procedure {\sf TBC-SC\_ComputeBound}} \{ \\
                        \> {\bf Input:} a set of valid worker-and-task pairs $S$, and a node $o$\\
                        \> {\bf Output:} the upper bound, $upperBound$, of the total quality score of node $o$\\
                        \> (1) \> \> $H_c = \emptyset$ //a max-heap w.r.t. to the quality rates of the pairs stored in it\\
                        \> (2) \> \> $upperBound = o.score$\\
                        \> (3) \> \> $remainBudget = o.budget$\\
                        \> (4) \> \> obtain a set of worker-and-task pairs of unexploited tasks and available \\
                        \> \> \> \>\> workers from $S$ and store them into $H_c$\\
                        \> (5) \> \> \textbf{while} $H_c$ is not empty\\
                        \> (6) \> \> \> $\langle w_i, t_j\rangle$ = $H_c$.pop()\\
                        \> (7) \> \> \> \textbf{if} $remainBudget > c_{ij}$\\
                        \> (8) \> \> \> \> $upperBound = upperBound + q_{ij}$\\
                        \> (9) \> \> \> \> $remainBudget = remainBudget - c_{ij}$\\
                        \> (10) \> \> \> \textbf{else} \\
                         \> (11) \> \> \> \> $upperBound = upperBound + q_{ij}\cdot (remainBudget/c_{ij})$\\
                        \> (12) \> \> \> \> $remainBudget = 0$\\
                        \> (13) \> \> \> \> \textbf{break}\\
                        \> (14) \> \>  \textbf{return} $upperBound$\\
                        \}
                    \end{tabbing}
                \end{scriptsize}
            }
        \end{tabular}
    \end{center}\vspace{-8ex}
    \caption{\small The Bounding Algorithm.}
    \vspace{-3ex}
    \label{alg:bb_bound}
\end{figure}

Figure \ref{alg:bb_bound} presents the pseudo code of our TBC-SC bounding
algorithm, namely TBC-SC\_ComputeBound, which efficiently estimates a tight upper
bound of the total quality score for a given node $o$. We first initialize the
max-heap w.r.t. the quality rates of the stored pairs, $H_c$, as an
empty set, the current upper bound value, $upperBound$,
as that of node $o$ and the remaining budget, $remainBudget$, as that of
node $o$ (lines 1-3). Then, we obtain the worker-and-task pairs $\langle w_i, t_j\rangle$
of unexploited tasks and available workers, where worker $w_i$ has not been
assigned to any tasks in previous levels and task $t_j$ has not been exploited (line 4).

Next, in each iteration, we greedily select one worker-and-task pair
$\langle w_i, t_j\rangle$ from $H_c$ and update the estimated upper
bound of the total quality score and the remaining budget (lines 5-13).
Specifically, if the remaining budget, $remainBudget$, is smaller than the
cost $c_{ij}$ of the selected worker-and-task pair $\langle w_i, t_j\rangle$ in the
current iteration, we add a portion of the quality score $q_{ij}$ to the estimated
upper bound according to the ratio of the remaining budget and the travel cost $c_{ij}$ (line 11).

Finally, we return the estimated upper bound of
the total quality score of node $o$ (line 17).



\begin{theorem}
    (Correctness of the Bounding Algorithm) Our proposed bounding algorithm can correctly return a upper bound of a given node $o$.
\end{theorem}
\begin{proof}
    We note $I$ as the set of selected pairs in lines 7-13 in Figure \ref{alg:bb_bound}. Assume this is another set of pairs $I' \subseteq H_c$ that can achieve higher quality score than the set $I$. That is:
    {\scriptsize\begin{equation}
    \sum_{\langle w'_i, t'_j\rangle \in I'}q'_{ij} > \sum_{\langle w_i, t_j\rangle \in I}q_{ij}\notag
    \end{equation} }
    Let the set of exclusively existing pairs of $I$ as $I^- = I/I'$. Similarly, let $I'^- = I'/I$.
    As the remaining budget $B$ is same for $I$ and $I'$, then we have
    {\scriptsize\begin{equation}
    \sum_{\langle w'_i, t'_j\rangle \in I'}c'_{ij} = \sum_{\langle w_i, t_j\rangle \in I}c_{ij}\notag
    \end{equation} }
    Assume worker-and-task pair $\langle w'_a, t'_b\rangle$ has the highest quality rate in $I'^-$ and worker-and-task pair $\langle w_a, t_b\rangle$ has the lowest quality rate in $I^-$. As we greedily select pairs with highest quality rates in our bounding algorithm (lines 5-13 in Figure \ref{alg:bb_bound}), we have the quality rate $qr_{ab}$ of $\langle w_a, t_b\rangle$ is higher than that $qr'_{ab}$ of $\langle w'_a, t'_b\rangle$. Then, we have
    {\scriptsize\begin{flalign}
    \sum_{\langle w_i, t_j\rangle \in I}q_{ij} &= \sum_{\langle w_i, t_j\rangle \in I\cap I'}q_{ij} + \sum_{\langle w_i, t_j\rangle \in I^-}q_{ij}\notag\\
    &\geq \sum_{\langle w_i, t_j\rangle \in I\cap I'}q_{ij} + \sum_{\langle w_i, t_j\rangle \in I^-}qr_{ab}\cdot c_{ij}\notag\\
    &= \sum_{\langle w_i, t_j\rangle \in I\cap I'}q_{ij} + qr_{ab}\cdot\sum_{\langle w_i, t_j\rangle \in I^-} c_{ij}\notag\\
    &\geq \sum_{\langle w_i, t_j\rangle \in I\cap I'}q_{ij} + qr'_{ab}\cdot\sum_{\langle w_i, t_j\rangle \in I'^-} c_{ij}\notag\\
    &\geq \sum_{\langle w_i, t_j\rangle \in I\cap I'}q_{ij} + \sum_{\langle w_i, t_j\rangle \in I'^-} q'_{ij}\notag\\
    &=\sum_{\langle w'_i, t'_j\rangle \in I'}q'_{ij}.\notag
    \end{flalign} }
This result conflicts with the assumption, thus $I'$ could not exist. This theorem is proved.
\end{proof}

\subsection{The Branch-and-Bound Algorithm}
In this subsection, we combine the branching/bounding algorithms to form a
branch-and-bound algorithm for our TBC-SC problem, namely TBC-SC\_BB. The
basic idea is to greedily improve the best known quality score such that the
inefficient nodes can be pruned quickly.

\begin{figure}[ht]
    \begin{center}
        \begin{tabular}{l}
            \parbox{3.1in}{
                \begin{scriptsize} \vspace{-4ex}
                    \begin{tabbing}
                        12\=12\=12\=12\=12\=12\=12\=12\=12\=12\=12\=\kill
                        {\bf Procedure {\sf TBC-SC\_BB}} \{ \\
                        \> {\bf Input:} $n$ workers in $W_p$, and $m$ time-constrained spatial tasks in $T_p$\\
                        \> {\bf Output:} a worker-and-task assignment instance set, $I_p$\\
                        \> (1) \> \> $bestScore = -1$ // the current best total quality score\\
                        \> (2) \> \> obtain a set, $S$, of valid worker-and-task pairs\\
                        \> (3) \> \> push the root node $ro$ into max-heap $H$ w.r.t. the upper bound values\\
                        \> (4) \> \> \textbf{while} $H$ is not empty\\
                        \> (5) \> \> \> $o$ = $H$.pop()\\
                        \> (6) \> \> \> \textbf{if} $o.upperBound \leq bestScore$\\
                        \> (7) \> \> \> \> prune node $o$ and \textbf{continue}\\
                        \> (8) \> \> \>  \textbf{while} $o$ is expandable\\
                        \> (9) \> \> \> \> $O$ = TBC-SC\_Expand($o$, $S$)\\
                        \> (10) \> \> \> \> \textbf{foreach} node $o'$ in $O$\\
                        \> (11) \> \> \> \> \> $o'.upperBound$ = TBC-SC\_ComputeBound($o'$, $S$) \\
                        \> (12) \> \> \> \> \> \textbf{if} $o'.upperBound$ > $bestScore$\\
                        \> (13) \> \> \> \> \> \> $H$.push($o'$)\\
                        \> (14) \> \> \> \> \> \textbf{else}\\
                        \> (15) \> \> \> \> \> \> prune node $o'$ from $O$\\
                        \> (16) \> \> \> \>   set $o$ as the node with highest upper bound of the remaining nodes in $O$\\
                        \> (17) \> \> \>  \textbf{if} $o.score$ > $bestScore$\\
                        \> (18) \> \> \> \>  $bestScore$ = $o.score$\\
                        \> (19) \> \> \> \>  $I_p$ = $o.I$\\
                        \> (20) \> \>  \textbf{return} $I_p$\\
                        \}
                    \end{tabbing}
                \end{scriptsize}
            }
        \end{tabular}
    \end{center}\vspace{-8ex}
    \caption{\small The Branch-and-Bound Algorithm.}
    \vspace{-1ex}
    \label{alg:bb}
\end{figure}

Specifically, in Algorithm TBC-SC\_BB, we first initialize the current known
best quality score as $-1$ (line 1). Then, we find out all valid worker-and-task
pairs $\langle w_i, t_j\rangle$ in the spatial crowdsourcing system at timestamp
$p$ (line 1). Here, the validity of pair $\langle w_i, t_j\rangle$ satisfies 2 conditions:
(1) worker $w_i$ can arrive at the location, $l_j$, of task $t_j$ before the arrival
deadline $e_j$; (2) the cost $c_{ij}$ is smaller than the global budget $B$.

Next, we push the root node $ro$ into a max-heap $H$, which maintains the
nodes in it and can pop out a node with highest upper bound value quickly
at each time. Here, the root node $ro$ is initialized as follow:
$$\begin{array}{ll}
    ro.score &= 0,\\
    ro.upperBound &= 0,\\
    ro.I &= \emptyset,\\
    ro.taskIndex &= 0,\\
    ro.budget &=B.
\end{array}$$

Then, for each iteration, we exploit one possible assignment strategy and
try to improve the best known quality score, $bestScore$, (lines 5-19).
Specifically, in each iteration, we pop one node with the highest upper bound
of the nodes in the max-heap $H$ and note it as $o$ (line 5). Then, if $bestScore$
is higher than the upper bound quality score of node $o$, we can safely prune
node $o$ and continue to conduct the next iteration (lines 6-7). Otherwise, we greedily
expand the current node $o$ and select the child node with highest upper bound
to iteratively exploit until it cannot be expanded (lines 8-16). Here, we use our
TBC-SC\_Expand algorithm to expand node $o$ in line 9. For the returned child
nodes, we use our TBC-SC\_ComputeBound to estimate the upper bound of quality
score for each child node $o'$ (line 11). For a child node $o'$, if its estimated upper
bound of quality score is higher than the best know quality score, it will be pushed
into the max-heap $H$; otherwise, it will be pruned from the set of child nodes $O$
(lines 12-15). When the inner iteration from line 8 to line 16 finished, we can
reach a node $o$ indicating a possible assignment strategy.
If this newly exploited assignment strategy can improve the best known quality score,
we update $bestScore$ and the set of worker-and-task pairs $I_p$ according to the
corresponding properties, $score$ and $I$, of node $o$ (lines 17-19).

Finally, we return the worker-and-task pairs $I_p$ with the exact highest quality score (line 20).

